Embedded domain Reduced Basis Models for the shallow water hyperbolic equations with the Shifted Boundary Method

We consider fully discrete embedded finite element approximations for a shallow water hyperbolic problem and its reduced-order model. Our approach is based on a fixed background mesh and an embedded reduced basis. The Shifted Boundary Method for spatial discretization is combined with an explicit predictor/multi-corrector time integration to integrate in time the numerical solutions to the shallow water equations, both for the full and reduced-order model. In order to improve the approximation of the solution manifold also for geometries that are untested during the offline stage, the snapshots have been pre-processed by means of an interpolation procedure that precedes the reduced basis computation. The methodology is tested on geometrically parametrized shapes with varying size and position.

==> section_hifi.tex <==
%!TEX root = main_cmame.tex
\begin{figure}[ht]\centering
%\begin{center}
\begin{minipage}{0.495\textwidth}
\includegraphics[width=1\textwidth]{figEK/H_HiFi0_5.png}
\end{minipage}
%\hskip 1cm
%\begin{minipage}{0.29\textwidth}
%\includegraphics[width=1\textwidth]{figEK/H_HiFi0_7.png}
%\end{minipage}
%\hskip -3.4cm
\begin{minipage}{0.495\textwidth}
\includegraphics[width=1\textwidth]{figEK/H_HiFi1_1.png}
\end{minipage}
\newline
%\begin{minipage}{0.26\textwidth}
%\includegraphics[width=1\textwidth]{figEK/H_HiFi1_3.png}
%\end{minipage}
%\hskip 1cm
%\begin{minipage}{0.26\textwidth}
%\includegraphics[width=1\textwidth]{figEK/H_HiFi1_5.png}
%\end{minipage}
%\hskip -3.4cm
\begin{minipage}{0.495\textwidth}
\includegraphics[width=1\textwidth]{figEK/H_HiFi1_7.png}
\end{minipage}
%
%\begin{minipage}{0.26\textwidth}
%\includegraphics[width=1\textwidth]{figEK/H_HiFi1_9.png}
%\end{minipage}
%
%\begin{minipage}{0.26\textwidth}
%\includegraphics[width=1\textwidth]{figEK/H_HiFi2_1.png}
%\end{minipage}
%\hskip 1cm
%\begin{minipage}{0.26\textwidth}
%\includegraphics[width=1\textwidth]{figEK/H_HiFi2_3.png}
%\end{minipage}
\begin{minipage}{0.495\textwidth}
\includegraphics[width=1\textwidth]{figEK/H_HiFi2_5.png}
\end{minipage}
%\end{center}
\caption{Snapshots with radius as parameter, and for $\mu=0.5$,  $1.1$, $1.7$,  $2.5$. We illustrate the height at final time $T=t=0.8$.}
\label{fig:snapshots_parametrized_Height}
\end{figure}

We parametrize the embedded geometry and in Figure \ref{fig:snapshots_parametrized_Height}, Figure \ref{fig:snapshots_parametrized_Velocity} we illustrate some snapshots for the height and the velocity X, Y, magnitude components with parameter the radius of the embedded circle. We visualize for parameter values  $\mu=0.5$,  $1.1$, $1.7$,  $2.5$.
%
\begin{figure}[ht]\centering
%%\begin{center}
%\begin{minipage}{0.495\textwidth}
%\includegraphics[width=1\textwidth]{figEK/VX_HiFi0_5.png}
%\end{minipage}
%%\hskip 1cm
%%\begin{minipage}{0.26\textwidth}
%%\includegraphics[width=1\textwidth]{figEK/VX_HiFi0_7.png}
%%\end{minipage}
%%\hskip -3.4cm
%\begin{minipage}{0.495\textwidth}
%\includegraphics[width=1\textwidth]{figEK/VX_HiFi1_1.png}
%\end{minipage}
%%
%%\begin{minipage}{0.26\textwidth}
%%\includegraphics[width=1\textwidth]{figEK/VX_HiFi1_3.png}
%%\end{minipage}
%%%\hskip 1cm
%%\begin{minipage}{0.26\textwidth}
%%\includegraphics[width=1\textwidth]{figEK/VX_HiFi1_5.png}
%%\end{minipage}
%%\hskip -3.4cm
%\begin{minipage}{0.495\textwidth}
%\includegraphics[width=1\textwidth]{figEK/VX_HiFi1_7.png}
%\end{minipage}
%%
%%\begin{minipage}{0.26\textwidth}
%%\includegraphics[width=1\textwidth]{figEK/VX_HiFi1_9.png}
%%\end{minipage}
%%
%%\begin{minipage}{0.26\textwidth}
%%\includegraphics[width=1\textwidth]{figEK/VX_HiFi2_1.png}
%%\end{minipage}
%%\hskip 1cm
%%\begin{minipage}{0.26\textwidth}
%%\includegraphics[width=1\textwidth]{figEK/VX_HiFi2_3.png}
%%\end{minipage}
%\begin{minipage}{0.495\textwidth}
%\includegraphics[width=1\textwidth]{figEK/VX_HiFi2_5.png}
%\end{minipage}
%\\
%\begin{minipage}{0.495\textwidth}
%\includegraphics[width=1\textwidth]{figEK/VY_HiFi0_5.png}
%\end{minipage}
%%\hskip 1cm
%%\begin{minipage}{0.26\textwidth}
%%\includegraphics[width=1\textwidth]{figEK/VY_HiFi0_7.png}
%%\end{minipage}
%%\hskip -3.4cm
%\begin{minipage}{0.495\textwidth}
%\includegraphics[width=1\textwidth]{figEK/VY_HiFi1_1.png}
%\end{minipage}
%%
%%\begin{minipage}{0.26\textwidth}
%%\includegraphics[width=1\textwidth]{figEK/VY_HiFi1_3.png}
%%\end{minipage}
%%\hskip 1cm
%%\begin{minipage}{0.26\textwidth}
%%\includegraphics[width=1\textwidth]{figEK/VY_HiFi1_5.png}
%%\end{minipage}
%%\hskip -3.4cm
%\begin{minipage}{0.495\textwidth}
%\includegraphics[width=1\textwidth]{figEK/VY_HiFi1_7.png}
%\end{minipage}
%%
%%\begin{minipage}{0.26\textwidth}
%%\includegraphics[width=1\textwidth]{figEK/VY_HiFi1_9.png}
%%\end{minipage}
%%
%%\begin{minipage}{0.26\textwidth}
%%\includegraphics[width=1\textwidth]{figEK/VY_HiFi2_1.png}
%%\end{minipage}
%%\hskip 1cm
%%\begin{minipage}{0.26\textwidth}
%\includegraphics[width=1\textwidth]{figEK/VY_HiFi2_3.png}
%%\end{minipage}
%\begin{minipage}{0.495\textwidth}
%\includegraphics[width=1\textwidth]{figEK/VY_HiFi2_5.png}
%\end{minipage}
%\\
\begin{minipage}{0.495\textwidth}
\includegraphics[width=1\textwidth]{figEK/V_HiFi0_5.png}
\end{minipage}
%\hskip 1cm
%\begin{minipage}{0.26\textwidth}
%\includegraphics[width=1\textwidth]{figEK/V_HiFi0_7.png}
%\end{minipage}
%\hskip -3.4cm
\begin{minipage}{0.495\textwidth}
\includegraphics[width=1\textwidth]{figEK/V_HiFi1_1.png}
\end{minipage}
%
%\begin{minipage}{0.26\textwidth}
%\includegraphics[width=1\textwidth]{figEK/V_HiFi1_3.png}
%\end{minipage}
%\hskip 1cm
%\begin{minipage}{0.26\textwidth}
%\includegraphics[width=1\textwidth]{figEK/V_HiFi1_5.png}
%\end{minipage}
%\hskip -3.4cm
\begin{minipage}{0.495\textwidth}
\includegraphics[width=1\textwidth]{figEK/V_HiFi1_7.png}
\end{minipage}
%
%\begin{minipage}{0.26\textwidth}
%\includegraphics[width=1\textwidth]{figEK/V_HiFi1_9.png}
%\end{minipage}
%
%\begin{minipage}{0.26\textwidth}
%\includegraphics[width=1\textwidth]{figEK/V_HiFi2_1.png}
%\end{minipage}
%\hskip 1cm
%\begin{minipage}{0.26\textwidth}
%\includegraphics[width=1\textwidth]{figEK/V_HiFi2_3.png}
%\end{minipage}
\begin{minipage}{0.495\textwidth}
\includegraphics[width=1\textwidth]{figEK/V_HiFi2_5.png}
\end{minipage}
%\end{center}
\caption{Snapshots with radius as parameter, and for $\mu=0.5$,  $1.1$,   $1.7$,  $2.5$. We illustrate the  the velocity X, Y, magnitude components at final time $T=t=0.8$.}
\label{fig:snapshots_parametrized_Velocity}
\end{figure}
%
